Homomorphic Encryption for Speaker Recognition: Protection of Biometric Templates and Vendor Model Parameters

Data privacy is crucial when dealing with biometric data. Accounting for the latest European data privacy regulation and payment service directive, biometric template protection is essential for any commercial application. Ensuring unlinkability across biometric service operators, irreversibility of leaked encrypted templates, and renewability of e.g., voice models following the i-vector paradigm, biometric voice-based systems are prepared for the latest EU data privacy legislation. Employing Paillier cryptosystems, Euclidean and cosine comparators are known to ensure data privacy demands, without loss of discrimination nor calibration performance. Bridging gaps from template protection to speaker recognition, two architectures are proposed for the two-covariance comparator, serving as a generative model in this study. The first architecture preserves privacy of biometric data capture subjects. In the second architecture, model parameters of the comparator are encrypted as well, such that biometric service providers can supply the same comparison modules employing different key pairs to multiple biometric service operators. An experimental proof-of-concept and complexity analysis is carried out on the data from the 2013-2014 NIST i-vector machine learning challenge.

==> figures/HE_2Cov/det_HE2Cov_new.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.75\detsize,
height=\detsize,
at={(0\detsize,0\detsize)},
scale only axis,
xmin=-5.61200124426585,
xmax=2.32634787404084,
xtick={-5.19933758218747,-4.75342430882831,-4.2648907939226,-3.71901648545571,-3.09023230616781,-2.32634787404084,-1.64485362695147,-1.03643338949379,-0.2533471031358,0.385320466407568,1.03643338949379,1.64485362695147},
xticklabels={{1e-5},{1e-4},{1e-3},{1e-2},{1e-1},{  1},{  5},{ 15},{ 40},{ 65},{ 85},{ 95}},
xlabel style={font=\color{white!15!black}},
xlabel={False Match Rate (in \%)},
ymin=-5.61200124426585,
ymax=2.32634787404084,
ytick={-5.19933758218747,-4.75342430882831,-4.2648907939226,-3.71901648545571,-3.09023230616781,-2.32634787404084,-1.64485362695147,-1.03643338949379,-0.2533471031358,0.385320466407568,1.03643338949379,1.64485362695147},
yticklabels={{1e-5},{1e-4},{1e-3},{1e-2},{1e-1},{  1},{  5},{ 15},{ 40},{ 65},{ 85},{ 95}},
ylabel style={font=\color{white!15!black}},
ylabel={False Non-Match Rate (in \%)},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids
]
\addplot [color=blue, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
0.711083720338787	-5.61200124426585\\
0.703803028192223	-4.45431603298565\\
0.69655945394473	-4.30349833447359\\
0.682180666780935	-4.14755536305337\\
0.667941558302678	-4.05377990866255\\
0.653836608223446	-3.98602708686972\\
0.632919292238579	-3.90978799201934\\
0.612275314758042	-3.85114787759998\\
0.585148336985948	-3.78917255286195\\
0.558445310062872	-3.7390264059859\\
0.525614916641245	-3.68722279365476\\
0.48694920042067	-3.63582585178159\\
0.442737020300349	-3.5859415199833\\
0.393242093345543	-3.53808973066376\\
0.338683072761799	-3.49245734923576\\
0.279215570778995	-3.44905165464377\\
0.214915261302607	-3.40778854882349\\
0.140033455002931	-3.36549460560776\\
0.0886735314089968	-3.33938847821547\\
0.0301285073399118	-3.29793942011581\\
-0.0356212826941604	-3.25721672290568\\
-0.0941863332424937	-3.22506383179689\\
-0.134780834722292	-3.17737525113525\\
-0.175598758891826	-3.13597357761711\\
-0.223597470531699	-3.0936163574694\\
-0.279098514596338	-3.05115916442131\\
-0.335473523357753	-3.01357831060996\\
-0.400207160083937	-2.97583561819216\\
-0.474171934689097	-2.93834011170448\\
-0.550829340661019	-2.90456980532354\\
-0.639094636509832	-2.87088848148377\\
-0.732649767277996	-2.84017945631218\\
-0.833109867410812	-2.81193579104219\\
-0.861986806375481	-2.80460782910334\\
-0.902296920822214	-2.76138560999871\\
-0.946376855767147	-2.72085482538623\\
-0.994732233515533	-2.68262036974841\\
-1.04801980479209	-2.64637236669414\\
-1.09394066398762	-2.61910344339323\\
-1.14585117666682	-2.58226982098602\\
-1.20272758675226	-2.54769160053124\\
-1.25656932268711	-2.51942020993217\\
-1.30456136679127	-2.49503534467623\\
-1.34753299621268	-2.46102932268481\\
-1.39832629097067	-2.42484648152113\\
-1.40623230623411	-2.41970352994258\\
-1.43478387220451	-2.40049764798254\\
-1.4681356548633	-2.35602102070034\\
-1.48054020422903	-2.33946263984411\\
-1.51874468540736	-2.293744035899\\
-1.5593041564648	-2.25236986435011\\
-1.60260430444883	-2.21452607179282\\
-1.65182835896021	-2.1777473304902\\
-1.70541502131932	-2.14369797113477\\
-1.7295204069986	-2.13007517822073\\
-1.76378996891901	-2.1101589348203\\
-1.77461680979326	-2.10050661975826\\
-1.81846359173814	-2.06091130114784\\
-1.86611388795211	-2.02430570532585\\
-1.90634101301973	-1.99760163684308\\
-1.95687487903576	-1.96345973099343\\
-1.96786710145179	-1.95674179162691\\
-1.97338871925915	-1.95318524305781\\
-1.98325468886287	-1.94614537319425\\
-2.02150066663713	-1.90219813868009\\
-2.06295463061771	-1.86164438519168\\
-2.10828997675263	-1.82393956686036\\
-2.11427207092146	-1.81940472667772\\
-2.14850242993381	-1.79516105349946\\
-2.19066208118316	-1.75942435857477\\
-2.23563391995393	-1.72347486441004\\
-2.28389547864595	-1.68896644446797\\
-2.29298965820305	-1.68308125926818\\
-2.2957915205229	-1.68091628071421\\
-2.3387502494157	-1.64229459238362\\
-2.35761381069066	-1.62720119293453\\
-2.39995611940729	-1.58856847352885\\
-2.40181671951287	-1.58700948962472\\
-2.44491471150017	-1.54908952135519\\
-2.46687734401168	-1.5319905404204\\
-2.50990691763978	-1.49366009488395\\
-2.52142834333241	-1.48441290865132\\
-2.55750046469746	-1.45649407147245\\
-2.57971638719187	-1.43997647308127\\
-2.59794207972589	-1.42529408852759\\
-2.63448944424639	-1.39542296821551\\
-2.63925494802893	-1.39125611956164\\
-2.6475396644321	-1.38299412710064\\
-2.67743170314654	-1.35085391453315\\
-2.71314457381577	-1.31129976684819\\
-2.75105940974723	-1.26513527981229\\
-2.77038930989124	-1.24235450514004\\
-2.7827133462277	-1.22768991923831\\
-2.82218628936149	-1.18520554503088\\
-2.84114977069717	-1.1600910079529\\
-2.87914716405686	-1.11431811750337\\
-2.88218196809152	-1.11096665248232\\
-2.92233967075797	-1.06836290535678\\
-2.96412130750983	-1.03068871642079\\
-2.96684901320048	-1.02800757674583\\
-2.97389107253791	-1.02089373879666\\
-2.98443861332364	-1.00944266722813\\
-3.00029551144309	-0.992940656991047\\
-3.03674123764719	-0.949926788027115\\
-3.07611181836	-0.905434781129974\\
-3.11786486611875	-0.865349139942793\\
-3.12711561372174	-0.857320391221782\\
-3.14287604048361	-0.841471288611432\\
-3.18396426167568	-0.800593666425581\\
-3.18677795408358	-0.798030028223219\\
-3.19069668577574	-0.793696812491084\\
-3.22943969714082	-0.748928860937813\\
-3.24676938481004	-0.731071442533522\\
-3.28694626467616	-0.687927019521226\\
-3.30160726992453	-0.67382934622919\\
-3.33889391339864	-0.630866796248183\\
-3.3412693917584	-0.628300834654308\\
-3.36240425384189	-0.604757629326187\\
-3.38649088561376	-0.579054385771097\\
-3.40539017810149	-0.560487541213439\\
-3.44248675420692	-0.506313710005021\\
-3.48115142502859	-0.458023791713788\\
-3.49093897002667	-0.446949062026105\\
-3.53084289915612	-0.400906906308068\\
-3.53842585890992	-0.392925542947157\\
-3.57662668360681	-0.339813950476484\\
-3.59854729679276	-0.312832318215706\\
-3.6395006897783	-0.259600274890302\\
-3.65533254895061	-0.239570407500119\\
-3.65719395189117	-0.236863889908469\\
-3.66068483042106	-0.231456034669725\\
-3.6771147114604	-0.206664299532751\\
-3.72162682592253	-0.133514201261817\\
-3.73946669056167	-0.098551295298634\\
-3.77662105606655	-0.0297008606520022\\
-3.79608656824266	0.0026308051701136\\
-3.80612560687733	0.0215742510100609\\
-3.84410155422953	0.100031824801907\\
-3.85452730542905	0.119723819112488\\
-3.89309258746397	0.20907297944957\\
-3.90439618838904	0.233077673432314\\
-3.94400320861465	0.31614932565446\\
-3.98509898608628	0.428102047457418\\
-3.99579488189188	0.455103993907598\\
-4.04020316553568	0.592647181550214\\
-4.08671787822734	0.72238342573659\\
-4.13120793549442	0.834743221444747\\
-4.18168794237825	0.95846257406621\\
-4.2326262296388	1.07154316505881\\
-4.24879326863111	1.10513384928719\\
-4.3083047590996	1.25353080780024\\
-4.37011877532748	1.39591068114307\\
-4.43069411778974	1.52488416048733\\
-4.49450712351185	1.65008636610269\\
-4.55824829478545	1.76446791533222\\
-4.61408782866178	1.85587152640674\\
-4.67497015500186	1.94600555608717\\
-4.72203287868246	2.00875246101942\\
-4.78264735875408	2.08057622422794\\
-4.83571207373942	2.13518879331662\\
-4.88809156197858	2.19508949196628\\
-4.93650152090255	2.24383025558291\\
-4.98364782504559	2.28531768747412\\
-5.03142501941748	2.32159205996647\\
-5.0382906911036	2.32634787404084\\
};
\addplot [color=red, forget plot]
  table[row sep=crcr]{%
-4.46625182412703	-5.61200124426585\\
-4.46625182412703	2.32634787404084\\
};
\addplot [color=green, forget plot]
  table[row sep=crcr]{%
-5.61200124426585	-2.49503534467623\\
2.32634787404084	-2.49503534467623\\
};
\end{axis}
\end{tikzpicture}%

==> preambles/config/General-config.tex <==
\usepackage[utf8]{inputenc}

\PassOptionsToPackage{T1}{fontenc} % T2A for cyrillics
	\usepackage{fontenc}    
	
\usepackage{etex}
%\overfullrule=1cm
\usepackage{fixme}
\newcommand{\todo}[1]{{\color{red}\textbf#1}\fxwarning{TODO: #1}} 


\PassOptionsToPackage{eulerchapternumbers,listings,%drafting,%
				 pdfspacing,%floatperchapter,%linedheaders,%
				 subfig,beramono,eulermath,parts,dottedtoc}{classicthesis}
				 
% ********************************************************************
% Triggers for this config
% ******************************************************************** 
\usepackage{ifthen}
\newboolean{enable-backrefs} % enable backrefs in the bibliography
\setboolean{enable-backrefs}{false} % true false
% ****************************************************************************************************

% ****************************************************************************************************
% 2. Personal data and user ad-hoc commands
% ****************************************************************************************************

\usepackage{color}
\definecolor{grau}{gray}{.66}
\definecolor{atip}{rgb}{0.043137,0.1843137,0.490196}
\definecolor{atip_grey}{rgb}{0.74117647,0.74117647,0.74117647}

% ********************************************************************
% Setup, finetuning, and useful commands
% ********************************************************************
\newcounter{dummy} % necessary for correct hyperlinks (to index, bib, etc.)
\newlength{\abcd} % for ab..z string length calculation
\providecommand{\mLyX}{L\kern-.1667em\lower.25em\hbox{Y}\kern-.125emX\@}
\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\Ie}{I.\,e.\xspace}
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\Eg}{E.\,g.\xspace} 
\newcommand{\fe}{f.\,e.\xspace} 
\newcommand{\Fe}{F.\,e.\xspace} 
\newcommand{\cf}{c.\,f.\xspace} 
\newcommand{\Cf}{C.\,f.\xspace} 
% ****************************************************************************************************

% ****************************************************************************************************
% 3. Loading some handy packages
% ****************************************************************************************************
% ******************************************************************** 
% Packages with options that might require adjustments
% ******************************************************************** 
\usepackage[british,ngerman]{babel}
\PassOptionsToPackage{square,numbers}{natbib}
\usepackage[sort]{natbib}
\PassOptionsToPackage{fleqn}{amsmath}		% math environments and more by the AMS 
\usepackage{amsmath}
\usepackage{array,amstext, amsfonts, amssymb, bm}
\usepackage{footnote}

% ******************************************************************** 
% General useful packages
% ******************************************************************** 
\usepackage{textcomp} % fix warning with missing font shapes
\usepackage{scrhack} % fix warnings when using KOMA with listings package          
\usepackage{xspace} % to get the spacing after macros right  
\usepackage{mparhack} % get marginpar right
\usepackage{fixltx2e} % fixes some LaTeX stuff 

%\PassOptionsToPackage{printonlyused,smaller,nohyperlinks}{acronym}
%\PassOptionsToPackage{printonlyused,smaller}{acronym}
%\usepackage{acronym} % nice macros for handling all acronyms in the thesis
%\renewcommand{\bflabel}[1]{{#1}\hfill} % fix the list of acronyms

%\usepackage[xindy]{glossaries} %use glossaries
% ****************************************************************************************************
% 4. Setup floats: tables, (sub)figures, and captions
% ****************************************************************************************************
\usepackage{tabularx} % better tables
	\setlength{\extrarowheight}{3pt} % increase table row height
\newcommand{\tableheadline}[1]{\multicolumn{1}{c}{\spacedlowsmallcaps{#1}}}
\newcommand{\myfloatalign}{\centering} % to be used with each float for alignment
\usepackage{caption}
\captionsetup{format=hang,font=small}
\usepackage{subfig}
% all figures to the section they belong
\usepackage[section]{placeins}
%\usepackage{subcaption} %
% ****************************************************************************************************

% ****************************************************************************************************
% 5. Setup code listings
% ****************************************************************************************************
\usepackage{listings} 
%\lstset{emph={trueIndex,root},emphstyle=\color{BlueViolet}}%\underbar} % for special keywords
\lstset{language=[LaTeX]Tex,%C++,
    keywordstyle=\color{RoyalBlue},%\bfseries,
    basicstyle=\small\ttfamily,
    %identifierstyle=\color{NavyBlue},
    commentstyle=\color{Green}\ttfamily,
    stringstyle=\rmfamily,
    numbers=none,%left,%
    numberstyle=\scriptsize,%\tiny
    stepnumber=5,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    frameround=ftff,
    frame=single,
    belowcaptionskip=.75\baselineskip
    %frame=L
} 
% ****************************************************************************************************    		   

% ****************************************************************************************************
% 6. PDFLaTeX, hyperreferences and citation backreferences
% ****************************************************************************************************
\PassOptionsToPackage{dvipsnames}{xcolor}
\usepackage{pgfplots}

%
\usetikzlibrary{external}
\tikzexternalize[mode=list and make, prefix=ext-tikz/]
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

%
%%\tikzset{external/system call={lulatex \tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname "\image" "\texsource"}}
%\tikzset{external/system call={pdflatex -halt-on-error -interaction=batchmode -jobname "\image" "\def\tikzexternalrealjob{Thesis}\input{Thesis}"}}
%\tikzsetexternalprefix{figures/cache/}

\pgfplotsset{compat=newest}
%\usetikzlibrary{plotmarks}
%\pgfplotsset{plot coordinates/math parser=false}
%\pgfplotsset{each nth point=100, filter discard warning=false, unbounded coords=discard}
%\pgfplotsset{every axis/.append style={%
    %scaled x ticks=false,
    %scaled y ticks=false%,
    %yticklabel style={/pgf/number format/.cd,fixed,fixed zerofill,precision=1},
    %xticklabel style={/pgf/number format/.cd,fixed,fixed zerofill,precision=2},
    %ytick={\pgfkeysvalueof{/pgfplots/ymax},\pgfkeysvalueof{/pgfplots/ymin}},
    %xtick={\pgfkeysvalueof{/pgfplots/xmax},\pgfkeysvalueof{/pgfplots/xmin}}
		%}}
%\usetikzlibrary{calc}
\newlength\figureheight
\newlength\figurewidth
%\usepgfplotslibrary[external]
%\tikzexternalize[shell escape=-enable-write18]
\usepackage{pgf}
\usepackage{pgffor}
\usepgflibrary{plothandlers}
\usepackage{pdfpages}
\usepackage[shortcuts]{extdash}

\usepackage[hyphens]{url} % linebreaks in URLs

\def\hyph{-\penalty0\hskip0pt\relax} % for hyphenations in word like surnames Wayne-Smith
% ********************************************************************
% Using PDFLaTeX
% ********************************************************************
\PassOptionsToPackage{pdftex,hyperfootnotes=false,pdfpagelabels}{hyperref}
	\usepackage{hyperref}  % backref linktocpage pagebackref
\pdfcompresslevel=9
\pdfadjustspacing=1 
\PassOptionsToPackage{pdftex}{graphicx}
	\usepackage{graphicx} 
% ********************************************************************
% Setup the style of the backrefs from the ography
% (translate the options to any language you use)
% ********************************************************************
\newcommand{\backrefnotcitedstring}{\relax}%(Not cited.)
\newcommand{\backrefcitedsinglestring}[1]{(Cited on page~#1.)}
\newcommand{\backrefcitedmultistring}[1]{(Cited on pages~#1.)}
\ifthenelse{\boolean{enable-backrefs}}%
{%
		\PassOptionsToPackage{hyperpageref}{backref}
		\usepackage{backref} % to be loaded after hyperref package 
		   \renewcommand{\backreftwosep}{ and~} % separate 2 pages
		   \renewcommand{\backreflastsep}{, and~} % separate last of longer list
		   \renewcommand*{\backref}[1]{}  % disable standard
		   \renewcommand*{\backrefalt}[4]{% detailed backref
		      \ifcase #1 %
		         \backrefnotcitedstring%
		      \or%
		         \backrefcitedsinglestring{#2}%
		      \else%
		         \backrefcitedmultistring{#2}%
		      \fi}%
}{\relax}    

% ****************************************************************************************************
% 7. Last calls before the bar closes
\usepackage{qtree}
\usepackage{siunitx} 

%Glossar, Abkürzungsverzeichnis, Symbolverzeichnis
\usepackage[style=long,nolist,acronym, nopostdot]{glossaries}
\makeglossaries
%\usepackage[nonumberlist, acronym, toc]{glossaries}

%Ein eigenes Symbolverzeichnis erstellen
%\newglossary[slg]{symbolslist}{syi}{syg}{List of symbols}

%Den Punkt am Ende jeder Beschreibung deaktivieren
%\renewcommand*{\glspostdescription}{}


%\usepackage[style=long,nolist]{glossaries} %use glossaries




%\newcommand*{\myglossaryindent}{0cm}

%\newglossarystyle{longwithindent}{%
%	\glossarystyle{long}%
%	\renewenvironment{theglossary}%
%	{\begin{longtable}[l]{@{\hspace{\myglossaryindent}}lp{\glsdescwidth}lp{\glspagelistwidth}@{}}}%
%		{\end{longtable}}%
%} 

%\glsdisablehyper

 %\usepackage[usenames,dvipsnames]{pstricks}
 \usepackage{epsfig}
 \usepackage{pst-grad} % For gradients
 \usepackage{pst-plot} % For axes

%Table
\usepackage{ragged2e}
\usepackage{array}
\usepackage{booktabs}

%TIKZ rotate
\newcommand{\rotateRPY}[3]% roll, pitch, yaw
{   \pgfmathsetmacro{\rollangle}{#1}
    \pgfmathsetmacro{\pitchangle}{#2}
    \pgfmathsetmacro{\yawangle}{#3}

    % to what vector is the x unit vector transformed, and which 2D vector is this?
    \pgfmathsetmacro{\newxx}{cos(\yawangle)*cos(\pitchangle)}
    \pgfmathsetmacro{\newxy}{sin(\yawangle)*cos(\pitchangle)}
    \pgfmathsetmacro{\newxz}{-sin(\pitchangle)}
    \path (\newxx,\newxy,\newxz);
    \pgfgetlastxy{\nxx}{\nxy};

    % to what vector is the y unit vector transformed, and which 2D vector is this?
    \pgfmathsetmacro{\newyx}{cos(\yawangle)*sin(\pitchangle)*sin(\rollangle)-sin(\yawangle)*cos(\rollangle)}
    \pgfmathsetmacro{\newyy}{sin(\yawangle)*sin(\pitchangle)*sin(\rollangle)+ cos(\yawangle)*cos(\rollangle)}
    \pgfmathsetmacro{\newyz}{cos(\pitchangle)*sin(\rollangle)}
    \path (\newyx,\newyy,\newyz);
    \pgfgetlastxy{\nyx}{\nyy};

    % to what vector is the z unit vector transformed, and which 2D vector is this?
    \pgfmathsetmacro{\newzx}{cos(\yawangle)*sin(\pitchangle)*cos(\rollangle)+ sin(\yawangle)*sin(\rollangle)}
    \pgfmathsetmacro{\newzy}{sin(\yawangle)*sin(\pitchangle)*cos(\rollangle)-cos(\yawangle)*sin(\rollangle)}
    \pgfmathsetmacro{\newzz}{cos(\pitchangle)*cos(\rollangle)}
    \path (\newzx,\newzy,\newzz);
    \pgfgetlastxy{\nzx}{\nzy};
}
\usetikzlibrary{3d}
\usetikzlibrary{calc}
\usetikzlibrary{arrows, decorations.markings, shapes.geometric}
\tikzset{RPY/.style={x={(\nxx,\nxy)},y={(\nyx,\nyy)},z={(\nzx,\nzy)}}}

% ****************************************************************************************************
% ********************************************************************
% Development Stuff
% ********************************************************************
\listfiles
%\PassOptionsToPackage{l2tabu,orthodox,abort}{nag}
%	\usepackage{nag}
%\PassOptionsToPackage{warning, all}{onlyamsmath}
%	\usepackage{onlyamsmath}
\usepackage{longtable,multirow}
\usepackage{arydshln}

% Column types
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

\usepackage[boxed]{algorithm2e}
% math abbreviations, f.e. FMR FNMR etc. as commands
%\input{math_abbreviations}
\usepackage[safe]{tipa}
\newcommand{\ipa}[1]{\textsl{\textipa{#1}}}
%\usepackage{tikzuml-v1.0b/tikz-uml}
\usepackage{dirtree}

%\usepackage[psfonts]{hiero}

% ********************************************************************
% Last, but not least...
% ********************************************************************
\usepackage{classicthesis} 
% ****************************************************************************************************



==> preambles/config/General-config_back.tex <==
%\PassOptionsToPackage{latin9}{inputenc}	% latin9 (ISO-8859-9) = latin1+"Euro sign"
\usepackage[utf8]{inputenc}
\PassOptionsToPackage{T1}{fontenc} % T2A for cyrillics
	\usepackage{fontenc}     

\usepackage{etex}
\overfullrule=1mm
\usepackage{fixme}
\newcommand{\todo}[1]{{\color{red}\textbf#1}\fxwarning{TODO: #1}}


% ****************************************************************************************************
% classicthesis-config.tex 
% formerly known as loadpackages.sty, classicthesis-ldpkg.sty, and classicthesis-preamble.sty 
% Use it at the beginning of your ClassicThesis.tex, or as a LaTeX Preamble 
% in your ClassicThesis.{tex,lyx} with \input{classicthesis-config}
% ****************************************************************************************************  
% If you like the classicthesis, then I would appreciate a postcard. 
% My address can be found in the file ClassicThesis.pdf. A collection 
% of the postcards I received so far is available online at 
% http://postcards.miede.de
% ****************************************************************************************************

% ****************************************************************************************************
% 1. Configure classicthesis for your needs here, e.g., remove "drafting" below 
% in order to deactivate the time-stamp on the pages
% ****************************************************************************************************
\PassOptionsToPackage{eulerchapternumbers,listings,%drafting,%
				 pdfspacing,%floatperchapter,%linedheaders,%
				 subfig,beramono,eulermath,parts,dottedtoc}{classicthesis}										
% ********************************************************************
% Available options for classicthesis.sty 
% (see ClassicThesis.pdf for more information):
% drafting
% parts nochapters linedheaders
% eulerchapternumbers beramono eulermath pdfspacing minionprospacing
% tocaligned dottedtoc manychapters
% listings floatperchapter subfig
% ********************************************************************

% ********************************************************************
% Triggers for this config
% ******************************************************************** 
\usepackage{ifthen}
\newboolean{enable-backrefs} % enable backrefs in the bibliography
\setboolean{enable-backrefs}{false} % true false
% ****************************************************************************************************


% ****************************************************************************************************
% 2. Personal data and user ad-hoc commands
% ****************************************************************************************************

\usepackage{color}
\definecolor{grau}{gray}{.66}
\definecolor{atip}{rgb}{0.043137,0.1843137,0.490196}
\definecolor{atip_grey}{rgb}{0.74117647,0.74117647,0.74117647}

% ********************************************************************
% Setup, finetuning, and useful commands
% ********************************************************************
\newcounter{dummy} % necessary for correct hyperlinks (to index, bib, etc.)
\newlength{\abcd} % for ab..z string length calculation
\providecommand{\mLyX}{L\kern-.1667em\lower.25em\hbox{Y}\kern-.125emX\@}
\newcommand{\ie}{i.\,e.\xspace}
\newcommand{\Ie}{I.\,e.\xspace}
\newcommand{\eg}{e.\,g.\xspace}
\newcommand{\Eg}{E.\,g.\xspace} 
\newcommand{\fe}{f.\,e.\xspace} 
\newcommand{\Fe}{F.\,e.\xspace} 
\newcommand{\cf}{c.\,f.\xspace} 
\newcommand{\Cf}{C.\,f.\xspace} 
% ****************************************************************************************************


% ****************************************************************************************************
% 3. Loading some handy packages
% ****************************************************************************************************
% ******************************************************************** 
% Packages with options that might require adjustments
% ******************************************************************** 

%\PassOptionsToPackage{ngerman,american}{babel}   % change this to your language(s)
% Spanish languages need extra options in order to work with this template
%\PassOptionsToPackage{spanish,es-lcroman}{babel}
 \usepackage[british,ngerman]{babel}
\PassOptionsToPackage{square,numbers}{natbib}
 \usepackage[sort]{natbib}
\PassOptionsToPackage{fleqn}{amsmath}		% math environments and more by the AMS 
 \usepackage{amsmath}
\usepackage{array,amstext, amsfonts, amssymb, bm}
\usepackage{footnote}
% ******************************************************************** 
% General useful packages
% ******************************************************************** 
\usepackage{textcomp} % fix warning with missing font shapes
\usepackage{scrhack} % fix warnings when using KOMA with listings package          
\usepackage{xspace} % to get the spacing after macros right  
\usepackage{mparhack} % get marginpar right
\usepackage{fixltx2e} % fixes some LaTeX stuff 
\PassOptionsToPackage{printonlyused,smaller}{acronym}
	\usepackage{acronym} % nice macros for handling all acronyms in the thesis
%\renewcommand*{\acsfont}[1]{\textssc{#1}} % for MinionPro
\renewcommand{\bflabel}[1]{{#1}\hfill} % fix the list of acronyms
% ****************************************************************************************************


% ****************************************************************************************************
% 4. Setup floats: tables, (sub)figures, and captions
% ****************************************************************************************************
\usepackage{tabularx} % better tables
	\setlength{\extrarowheight}{3pt} % increase table row height
\newcommand{\tableheadline}[1]{\multicolumn{1}{c}{\spacedlowsmallcaps{#1}}}
\newcommand{\myfloatalign}{\centering} % to be used with each float for alignment
\usepackage{caption}
\captionsetup{format=hang,font=small}
\usepackage{subfig}
% ****************************************************************************************************


% ****************************************************************************************************
% 5. Setup code listings
% ****************************************************************************************************
\usepackage{listings} 
%\lstset{emph={trueIndex,root},emphstyle=\color{BlueViolet}}%\underbar} % for special keywords
\lstset{language=[LaTeX]Tex,%C++,
    keywordstyle=\color{RoyalBlue},%\bfseries,
    basicstyle=\small\ttfamily,
    %identifierstyle=\color{NavyBlue},
    commentstyle=\color{Green}\ttfamily,
    stringstyle=\rmfamily,
    numbers=none,%left,%
    numberstyle=\scriptsize,%\tiny
    stepnumber=5,
    numbersep=8pt,
    showstringspaces=false,
    breaklines=true,
    frameround=ftff,
    frame=single,
    belowcaptionskip=.75\baselineskip
    %frame=L
} 
% ****************************************************************************************************    		   


% ****************************************************************************************************
% 6. PDFLaTeX, hyperreferences and citation backreferences
% ****************************************************************************************************
\PassOptionsToPackage{dvipsnames}{xcolor}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
%\usetikzlibrary{plotmarks}
%\pgfplotsset{plot coordinates/math parser=false}
%\pgfplotsset{each nth point=100, filter discard warning=false, unbounded coords=discard}
%\pgfplotsset{every axis/.append style={%
    %scaled x ticks=false,
    %scaled y ticks=false%,
    %yticklabel style={/pgf/number format/.cd,fixed,fixed zerofill,precision=1},
    %xticklabel style={/pgf/number format/.cd,fixed,fixed zerofill,precision=2},
    %ytick={\pgfkeysvalueof{/pgfplots/ymax},\pgfkeysvalueof{/pgfplots/ymin}},
    %xtick={\pgfkeysvalueof{/pgfplots/xmax},\pgfkeysvalueof{/pgfplots/xmin}}
		%}}
%\usetikzlibrary{calc}
\newlength\figureheight
\newlength\figurewidth
%\usepgfplotslibrary[external]
%\tikzexternalize[shell escape=-enable-write18]
\usepackage{pgf}
\usepackage{pgffor}
\usepgflibrary{plothandlers}
\usepackage{pdfpages}
\usepackage[shortcuts]{extdash}

\usepackage[hyphens]{url} % linebreaks in URLs

\def\hyph{-\penalty0\hskip0pt\relax} % for hyphenations in word like surnames Wayne-Smith
% ********************************************************************
% Using PDFLaTeX
% ********************************************************************
\PassOptionsToPackage{pdftex,hyperfootnotes=false,pdfpagelabels}{hyperref}
	\usepackage{hyperref}  % backref linktocpage pagebackref
\pdfcompresslevel=9
\pdfadjustspacing=1 
\PassOptionsToPackage{pdftex}{graphicx}
	\usepackage{graphicx} 

% ********************************************************************
% Setup the style of the backrefs from the bibliography
% (translate the options to any language you use)
% ********************************************************************
\newcommand{\backrefnotcitedstring}{\relax}%(Not cited.)
\newcommand{\backrefcitedsinglestring}[1]{(Cited on page~#1.)}
\newcommand{\backrefcitedmultistring}[1]{(Cited on pages~#1.)}
\ifthenelse{\boolean{enable-backrefs}}%
{%
		\PassOptionsToPackage{hyperpageref}{backref}
		\usepackage{backref} % to be loaded after hyperref package 
		   \renewcommand{\backreftwosep}{ and~} % separate 2 pages
		   \renewcommand{\backreflastsep}{, and~} % separate last of longer list
		   \renewcommand*{\backref}[1]{}  % disable standard
		   \renewcommand*{\backrefalt}[4]{% detailed backref
		      \ifcase #1 %
		         \backrefnotcitedstring%
		      \or%
		         \backrefcitedsinglestring{#2}%
		      \else%
		         \backrefcitedmultistring{#2}%
		      \fi}%
}{\relax}    


% ********************************************************************
% Setup autoreferences
% ********************************************************************
% There are some issues regarding autorefnames
% http://www.ureader.de/msg/136221647.aspx
% http://www.tex.ac.uk/cgi-bin/texfaq2html?label=latexwords
% you have to redefine the makros for the 
% language you use, e.g., american, ngerman
% (as chosen when loading babel/AtBeginDocument)
% ********************************************************************
%\makeatletter
%\@ifpackageloaded{babel}%
%    {%
%       \addto\extrasamerican{%
%					\renewcommand*{\figureautorefname}{Figure}%
%					\renewcommand*{\tableautorefname}{Table}%
%					\renewcommand*{\partautorefname}{Part}%
%					\renewcommand*{\chapterautorefname}{Chapter}%
%					\renewcommand*{\sectionautorefname}{Section}%
%					\renewcommand*{\subsectionautorefname}{Section}%
%					\renewcommand*{\subsubsectionautorefname}{Section}% 	
%				}%
%       \addto\extrasngerman{% 
%					\renewcommand*{\paragraphautorefname}{Absatz}%
%					\renewcommand*{\subparagraphautorefname}{Unterabsatz}%
%					\renewcommand*{\footnoteautorefname}{Fu\"snote}%
%					\renewcommand*{\FancyVerbLineautorefname}{Zeile}%
%					\renewcommand*{\theoremautorefname}{Theorem}%
%					\renewcommand*{\appendixautorefname}{Anhang}%
%					\renewcommand*{\equationautorefname}{Gleichung}%        
%					\renewcommand*{\itemautorefname}{Punkt}%
%				}%	
%			% Fix to getting autorefs for subfigures right (thanks to Belinda Vogt for changing the definition)
%			\providecommand{\subfigureautorefname}{\figureautorefname}%  			
%    }{\relax}
%\makeatother


% ****************************************************************************************************
% 7. Last calls before the bar closes

% ********************************************************************
% Using Glossary
% ********************************************************************
\usepackage[nonumberlist, toc]{glossaries}

% ****************************************************************************************************
% ********************************************************************
% Development Stuff
% ********************************************************************
\listfiles
%\PassOptionsToPackage{l2tabu,orthodox,abort}{nag}
%	\usepackage{nag}
%\PassOptionsToPackage{warning, all}{onlyamsmath}
%	\usepackage{onlyamsmath}
\usepackage{longtable,multirow}
\usepackage{arydshln}

% Column types
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

\usepackage[boxed]{algorithm2e}
% math abbreviations, f.e. FMR FNMR etc. as commands
%\input{math_abbreviations}
\usepackage[safe]{tipa}
\newcommand{\ipa}[1]{\textsl{\textipa{#1}}}
%\usepackage{tikzuml-v1.0b/tikz-uml}
\usepackage{dirtree}

%\usepackage[psfonts]{hiero}

% ********************************************************************
% Last, but not least...
% ********************************************************************
\usepackage{classicthesis} 
% ****************************************************************************************************

% ****************************************************************************************************
% 8. Further adjustments (experimental)
% ****************************************************************************************************
% Seitenzahlen math mode ... sieht nicht gut aus
%\lehead{\mbox{\llap{\small\(\scriptstyle\thepage\)\kern2em}\headmark\hfil}}
%\rohead{\mbox{\hfil{\headmark}\rlap{\small\kern2em\(\scriptstyle\thepage\)}}}

% ********************************************************************
% Changing the text area
% ********************************************************************
%\linespread{1.05} % a bit more for Palatino
%\areaset[current]{312pt}{761pt} % 686 (factor 2.2) + 33 head + 42 head \the\footskip
%\setlength{\marginparwidth}{7em}%
%\setlength{\marginparsep}{2em}%

% ********************************************************************
% Using different fonts
% ********************************************************************
%\usepackage[oldstylenums]{kpfonts} % oldstyle notextcomp
%\usepackage{hfoldsty} % Computer Modern with osf
%\usepackage[light,condensed,math]{iwona}
%\renewcommand{\sfdefault}{iwona}
%\usepackage{lmodern} % <-- no osf support :-(
%\usepackage[urw-garamond]{mathdesign} <-- no osf support :-(
% ****************************************************************************************************





==> preambles/config/Thesis-config.tex <==
% ********************************************************************
% Hyperreferences
% ********************************************************************
\hypersetup{%
    %draft,	% = no hyperlinking at all (useful in b/w printouts)
    colorlinks=true, linktocpage=true, pdfstartpage=3, pdfstartview=FitV,%
    % uncomment the following line if you want to have black links (e.g., for printing)
    %colorlinks=false, linktocpage=false, pdfborder={0 0 0}, pdfstartpage=3, pdfstartview=FitV,% 
    breaklinks=true, pdfpagemode=UseNone, pageanchor=true, pdfpagemode=UseOutlines,%
    plainpages=false, bookmarksnumbered, bookmarksopen=true, bookmarksopenlevel=1,%
    hypertexnames=true, pdfhighlight=/O,%nesting=true,%frenchlinks,%
    urlcolor=webbrown, linkcolor=RoyalBlue, citecolor=webgreen, %pagecolor=RoyalBlue,%
    %urlcolor=Black, linkcolor=Black, citecolor=Black, %pagecolor=Black,%
    pdftitle={\myTitle},%
    pdfauthor={\textcopyright\ \myName, \myUni},%
    pdfsubject={\mySubtitle},%
    pdfkeywords={\myKeywords},%
    pdfcreator={pdfLaTeX},%
    pdfproducer={LaTeX with hyperref and classicthesis}%
}

\newcommand{\titleleftmargin}{-1cm}
\newcommand{\titlerightmargin}{-3cm}

==> preambles/config/Thesis-config_online.tex <==
% ********************************************************************
% Hyperreferences
% ********************************************************************
\hypersetup{%
    %draft,	% = no hyperlinking at all (useful in b/w printouts)
    %colorlinks=true, linktocpage=true, pdfstartpage=1, pdfstartview=FitV,%
    % uncomment the following line if you want to have black links (e.g., for printing)
    colorlinks=true, linktocpage=false, pdfborder={0 0 0}, pdfstartpage=3, pdfstartview=FitV,% 
    breaklinks=true, pdfpagemode=UseNone, pageanchor=true, pdfpagemode=UseOutlines,%
    plainpages=false, bookmarksnumbered, bookmarksopen=true, bookmarksopenlevel=1,%
    hypertexnames=true, pdfhighlight=/O,%nesting=true,%frenchlinks,%
    %urlcolor=black, linkcolor=black, citecolor=black, %pagecolor=RoyalBlue,%
    urlcolor=webbrown, linkcolor=RoyalBlue, citecolor=webgreen, %pagecolor=RoyalBlue,%
    %urlcolor=Black, linkcolor=Black, citecolor=Black, %pagecolor=Black,%
    pdftitle={\myTitle},%
    pdfauthor={\textcopyright\ \myName, \myUni},%
    pdfsubject={\mySubtitle},%
    pdfkeywords={\myKeywords},%
    pdfcreator={pdfLaTeX},%
    pdfproducer={LaTeX with hyperref and classicthesis}%
}

\newcommand{\titleleftmargin}{0cm}
\newcommand{\titlerightmargin}{0cm}



==> preambles/config/myInfo.tex <==
\newcommand{\myTitle}{Presentation Attack Detection for State-of-the-Art Speaker Recognition Systems\xspace}
\newcommand{\mySubtitle}{Detection of Unit-Selection Attacks utilising Frequency Based Signal Analysis\xspace}
\newcommand{\myDegree}{Master of Science (M.Sc.)\xspace}
\newcommand{\myName}{Ulrich Johannes Scherhag\xspace}
\newcommand{\myProf}{Prof. Dr. Christoph Busch\xspace}
\newcommand{\myOtherProf}{Andreas Nautsch\xspace}
\newcommand{\myFaculty}{Faculty of Computer Science\xspace}
\newcommand{\myDepartment}{Biometrics and Internet-Security Research Group\xspace}
\newcommand{\myUni}{Hochschule Darmstadt, University of Applied Science\xspace}
\newcommand{\myLocation}{Darmstadt\xspace}
\newcommand{\startdate}{30.09.2015}
\newcommand{\duedate}{01.04.2016}
\newcommand{\myKeywords}{biometrics,speaker recognition,spoofing}

\newcommand{\myTime}{\today\xspace}



==> preambles/gantt.tex <==
%\documentclass[border=3mm,tikz,convert={density=300,size=16x9cm,outext=gantt-150707-isodate.png}]{standalone}

\usepackage{pgfgantt}
\usetikzlibrary{patterns,automata}

% customization for ganttbars exceeding LaTeX dimension limits
\usepackage{datenumber}
\usepackage{xstring}
\usepackage{calc}

\newcounter{dateone}
\newcounter{datetwo}
\newcount\dateprogress
\newcount\percprogress
\newcommand{\progressDay}{def}

\newcommand{\progressday}[3]{%
	% diff dates in days
	\StrMid{#1}{1}{4}[\yearA]
	\StrMid{#1}{6}{7}[\monthA]
	\StrMid{#1}{9}{10}[\dayA]
	\StrMid{#2}{1}{4}[\yearB]
	\StrMid{#2}{6}{7}[\monthB]
	\StrMid{#2}{9}{10}[\dayB]
	\setmydatenumber{dateone}{\yearA}{\monthA}{\dayA}%
	\setmydatenumber{datetwo}{\yearB}{\monthB}{\dayB}%
	\addtocounter{datetwo}{-\thedateone}%
	% %\the\numexpr\thedatetwo
	% progressed days
	\percprogress=#3
	\dateprogress=\value{datetwo}
	\multiply\dateprogress by \percprogress
	\divide\dateprogress by 100
	% %\number\dateprogress
	\advance\dateprogress by \value{dateone}
	\setcounter{dateone}{\dateprogress}
	% %\the\numexpr\thedateone
	\setdatebynumber{\value{dateone}}
	% %\datedate
	\renewcommand\progressDay{\thedateyear-\thedatemonth-\thedateday}
	\progressDay{}
	%\thedateyear-\thedatemonth-\thedateday
}

% creates 3 ganttbars with different colors
% - overall bar with name: #2
% - completed bar with name: #2start
% - todo bar with name: #2end
\newcommand{\ganttbariso}[6]{
	% Parameters as \ganttbar:
	% 1. title
	% 2. name
	% 3. progress
	% 4. start iso-date
	% 5. end iso-date
	% 6. progress placing as data e.g., max date
	
	% calculate iso-date of progress
	\IfStrEq{#3}{none}{
		\renewcommand{\progressDay}{#4}
	}{
		\progressday{#4}{#5}{#3}
	}
	
	% Position of progress
	\ganttbar[name=#2progress,progress=#3,bar/.append style={draw=none}]{#1}{#6+1}{#6}
	%\newcommand{\ganttname}{#2 (#3)}
	%\ganttbar[name=\ganttname,progress=#3]{#1}{#5}{#5}
	
	
	% fulfilled bar
	\ganttbar[progress=none,name=#2start,bar/.append style={fill=white}]{}{#4}{\progressDay}% entspricht 60 %
	%\draw ([yshift=-0.125pt]#2start.north west)--([yshift=0.25pt]#2start.south west)
	%      ([yshift=-0.125pt]#2start.north west)--([yshift=-0.125pt]#2start.north east)
	%      ([yshift=0.25pt]#2start.south west)--([yshift=0.25pt]#2start.south east);
	\IfStrEq{#3}{100}{
		\ganttbar[progress=none,name=#2,bar/.append style={fill=white}]{}{#4}{#5}
	}{
		\ganttbar[progress=none,name=#2,bar/.append style={fill=lightgray}]{}{\progressDay}{#5}
	}
	% todo bar
	%\draw ([yshift=-0.125pt,xshift=-0.25pt]#2end.north east)--([yshift=0.25pt,xshift=-0.25pt]#2end.south east)
	%      ([yshift=-0.125pt]#2end.north west)--([yshift=-0.125pt]#2end.north east)
	%      ([yshift=0.25pt]#2end.south west)--([yshift=0.25pt]#2end.south east);
	
	% optional: reset day counters
	%\setdatetoday
}

\setganttlinklabel{f-s}{}

\ganttset{
	hgrid, 
	x unit 							= 0.25mm, 
	y unit title 					= 8mm, 
	y unit chart 					= 8mm,
	milestone left shift 			= -5,
	milestone right shift 			= 5,
	milestone progress label node/.append style={anchor=north,yshift=-.75mm},
	link/.style={-stealth, thick,blue}, 
	time slot format=isodate,
	bar progress label node/.append style={xshift=1em}
}

\newganttchartelement*{document}{
	document/.style={
		/pgfgantt/progress=none,
		/pgfgantt/milestone,
		fill=white,shape=circle
	},
	document incomplete/.style={
		/pgfgantt/document
	}
}

\newganttchartelement*{meeting}{
	meeting/.style={
		/pgfgantt/progress=none,
		/pgfgantt/milestone,
		/pgfgantt/milestone/.append style={left shift=-16,right shift=16},
		fill=white,shape=rectangle,
	},
	meeting incomplete/.style={
		/pgfgantt/meeting
	}
}

\makeatletter
\newcommand*{\stripunit}[1]{\strip@pt#1}
\makeatother

% 2 arguments: start & end dates
\newcounter{startdateiso}
\newcounter{enddateiso}
\newcounter{numdaysdateiso}
\newlength{\dayunitmm}
\newlength{\ganttshiftlength}
\newcommand{\setGanttWidthByISOdatesCropMaxText}[3]{
	% diff dates in days
	\StrMid{#1}{1}{4}[\yearA]
	\StrMid{#1}{6}{7}[\monthA]
	\StrMid{#1}{9}{10}[\dayA]
	\StrMid{#2}{1}{4}[\yearB]
	\StrMid{#2}{6}{7}[\monthB]
	\StrMid{#2}{9}{10}[\dayB]
	\setmydatenumber{startdateiso}{\yearA}{\monthA}{\dayA}%
	\setmydatenumber{enddateiso}{\yearB}{\monthB}{\dayB}%
	\setmydatenumber{numdaysdateiso}{\yearB}{\monthB}{\dayB}%
	\addtocounter{numdaysdateiso}{-\thestartdateiso}%
	% 0.95 is a scaling factor, one may to change font size of #3 or add a few letters
	\setlength{\dayunitmm}{(\linewidth-\widthof{#3}-0.75em-1em-\widthof{\footnotesize 100\% complete})/\real{\value{numdaysdateiso}}*\real{0.95}}
	% \number returns sp --> mm
	% scaled point (65536 sp = 1 pt), millimeter (10 mm = 1 cm), centimeter (2.54 cm = 1 in), inch (1 in = 72.27 pt)
	% *\real{2.54}*\real{10}/\real{65536}/\real{72.27}
	\setlength{\ganttshiftlength}{5\dayunitmm}
	\addtolength{\ganttshiftlength}{1.5pt}
	% adjust Gantt x-labels
	% \the\dayunitmm
	% \stripunit{\ganttshiftlength}
	\ganttset{
		x unit = \dayunitmm
	}
}
\newcommand{\setGanttWidthByISOdates}[2]{
	\setGanttWidthByISOdatesCropMaxText{#1}{#2}{}
}


% ===========================
% ========= Example =========
% ===========================
\iffalse
\begin{document}
	\begin{tikzpicture}
		\begin{ganttchart}[
			today=2016-06-29,%progress=today
			]{2016-06-01}{2017-06-30}
			% Gantt-Chart Header
			\gantttitlecalendar{year,month}\\				
			% Documents supervision
			\ganttbar{Documents}{2016-06-01}{2017-06-30}
			\ganttdocument[inline,
				document inline label node/.append style={font=\scriptsize,above}
				]{Proposal}{2016-06-25}\\
			% Meetings
			\ganttbar{Meetings}{2016-06-01}{2017-06-30}
				\ganttmeeting[inline,
				meeting inline label node/.append style={font=\scriptsize,above},
				meeting left shift=-5,meeting right shift=5
				]{KickOff}{2016-07-04}\\
			% WP 1
			% \ganttbariso{title}{objName}{progress}{startDate}{endDate}
			\ganttbariso{Title XY (WP1)}{WP1}{10}{2016-06-01}{2016-12-31}\\
			% \ganttmilestone[name=objName,progress=%|none]{title}{date}
			\ganttmilestone[name=M1,progress=none]{M1: milestone name}{2016-10-31}\\
			% WP 2
			\ganttbariso{Ttile YZ (WP2)}{WP2}{none}{2017-01-01}{2017-06-30}
			% Dependencies
			\ganttlink[link type=dr]{M1}{WP2start}
			\ganttlink[link type=rdldr,
				link bulge=10,
				link/.style={->,color=orange,ultra thick}
				]{WP1}{WP2start}
			\ganttlink[link type=rdldr,
				link bulge=5,link mid=0.6,
				link/.style={->,color=darkgreen,ultra thick}
				]{WP1}{WP2start}
			\ganttlink[link type=f-s]{WP1}{WP2start}
		\end{ganttchart}
	\end{tikzpicture}
\end{document}
\fi

==> preambles/glossaries.tex <==
\usepackage[style=long,nolist,acronym, nopostdot]{glossaries}
\makeglossaries

% https://en.wikibooks.org/wiki/LaTeX/Glossary#Dual_entries_with_reference_to_a_glossary_entry_from_an_acronym
\DeclareDocumentCommand{\newdualentry}{ O{} O{} m m m m } {
	\newglossaryentry{gls-#3}{name={#5},text={#5\glsadd{#3}},
		description={#6},#1
	}
	\makeglossaries
	\newacronym[see={[Glossary:]{gls-#3}},#2]{#3}{#4}{#5\glsadd{gls-#3}}
}


==> preambles/href-thesis.tex <==
\PassOptionsToPackage{hyphens}{url}
\PassOptionsToPackage{pdftex,hyperfootnotes=false,pdfpagelabels}{hyperref}
\usepackage{hyperref}  % backref linktocpage pagebackref

==> preambles/ieee-spl.tex <==
% from IEEE template recommendation
\usepackage[T1]{fontenc} % optional
\usepackage{amsmath}
\usepackage[cmintegrals]{newtxmath}

==> preambles/packages-speech-tipa.tex <==
\usepackage[safe]{tipa}
\newcommand{\ipa}[1]{\textsl{\textipa{#1}}}

==> preambles/poster-header-dasec.tex <==

\begin{poster}% 5 arguments
{% --- key-values
 headerheight=6cm,
 grid=false,
 borderColor=bordercol, % Border color of content boxes
 headerColorOne=headercol1, % Background color for the header in the content boxes (left  side)
 headerColorTwo=headercol2, % Background color for the header in the content boxes (right side)
 headerFontColor=headerfontcol, % Text color for the header text in the content boxes
 boxColorOne=boxcolor, % Background color for the content in the content boxes
 headershape=rounded, % Specify the rounded corner in the content box headers
 headerfont=\Large\sf\bf, % Font modifiers for the text in the content box headers
 textborder=rounded,
 background=shadeTB,
 bgColorOne=white,
 bgColorTwo=gray!50,
 headerborder=open, % Change to closed for a line under the content box headers
 boxshade=plain,
 eyecatcher=true % Set to false for ignoring the left logo in the title and move the title left
}
{% --- eye catcher
%\vspace{1cm}
\bgroup\def\arraystretch{2}
 \begin{tabular}{c}\\[1.5cm]
   \paperlogos
 \end{tabular}
\egroup
}
{% --- title
\vspace{0.5cm}
\begin{minipage}{1.3\textwidth}
\hspace{-6.5cm}
\centering
{
\huge % usually \Huge by default
\textsc{\papertitle}
\vspace{2cm}
}
\end{minipage}
}
{% --- authors
\vspace{-1.25cm}
{\centering \textsc{\paperauthors}}\\[1em]
{	\small
	\papersites \\
	\small
	\texttt{\paperemails}
}
\vspace{0.25cm}
}
{% --- logos
\begin{tabular}{c}\\[2cm]
\hspace{2em}\includegraphics[width=0.1\paperwidth]{logos-dasec/hda_loewe_crisp_logos.pdf} 
\end{tabular}
}

==> preambles/poster.tex <==
\input{preambles/default.tex}

\renewcommand{\familydefault}{\sfdefault}
\pgfplotsset{grid style={dashed,gray}}
%\tikzset{ 
%	every plot/.style={prefix=plots/pgf-}, 
%	shape dasec/.style={ 
%		color=hda, 
%		draw,
%		fill=white,
%		line width=0.01cm,
%		minimum height=1.25em,
%		inner xsep=0.0cm,
%		inner ysep=0.0cm} 
%}
%
%\usepackage{xcolor}
%\usepackage[framemethod=TikZ]{mdframed}
%\mdfdefinestyle{MyFrame}{
%	linecolor=red,
%	outerlinewidth=6pt,
%	roundcorner=20pt,
%	innertopmargin=\baselineskip,
%	innerbottommargin=\baselineskip,
%	innerrightmargin=20pt,
%	innerleftmargin=20pt,
%	backgroundcolor=white!50!white}

\usepackage{epsfig}
\usepackage{float}
\usepackage{relsize} % Used for making text smaller in some places
%\usepackage{subfigure}

\newcommand{\compresslist}{ % Define a command to reduce spacing within itemize/enumerate environments, this is used right after \begin{itemize} or \begin{enumerate}
	\setlength{\itemsep}{1pt}
	\setlength{\parskip}{0pt}
	\setlength{\parsep}{0pt}
}

\definecolor{lightblue}{rgb}{0.145,0.6666,1} % Defines the color used for content box headers
\definecolor{bordercol}{RGB}{20,20,20} % Border color of content boxes
\definecolor{headercol1}{RGB}{240,240,240}%{255,200,200} % Background color for the header in the content boxes (left side)
\definecolor{headercol2}{RGB}{255,255,255} % Background color for the header in the content boxes (right side)
\definecolor{headerfontcol}{RGB}{0,0,0} % Text color for the header text in the content boxes
\definecolor{boxcolor}{RGB}{255, 255, 255} % Background color for the content in the content boxes
\definecolor{bgColorOne}{RGB}{200, 200, 200} % Background color for the content in the content boxes


==> preambles/thesis-layout-print.tex <==
\newcommand{\titleleftmargin}{-1cm}
\newcommand{\titlerightmargin}{-3cm}

==> preambles/thesis.tex <==
\usepackage{framed} % for thesis box

% Hand made theorem, see: https://en.wikibooks.org/wiki/LaTeX/Theorems
\usepackage{amsthm}
\usepackage{thmtools}
\theoremstyle{plain}
\newtheoremstyle{hypothesis}% name of the style to be used
    {3pt}% measure of space to leave above the theorem. E.g.: 3pt
    {3pt}% measure of space to leave below the theorem. E.g.: 3pt
    {\itshape}% name of font to use in the body of the theorem
    {2.5em}% measure of space to indent
    {\bfseries}% name of head font
    {}% punctuation between head and body
    { }% space after theorem head; " " = normal interword space
    {\thmname{#1}\thmnumber{ #2}:\thmnote{ #3}}% Manually specify head
\theoremstyle{hypothesis}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem*{hypothesis*}{Hypothesis}
% listing theorems, hypotheses
\makeatletter
\def\ll@hypothesis{%
    \protect\numberline{\thehypothesis}\thmt@shortoptarg%
}
\makeatother


\titleformat{\section}
{\raggedright}{\textsc{\MakeTextLowercase{\thesection}}}{1em}{\spacedlowsmallcaps}
\titleformat{\subsection}
{\raggedright}{\textsc{\MakeTextLowercase{\thesubsection}}}{1em}{\normalsize\itshape}
\titleformat{\subsubsection}
{\raggedright}{\textsc{\MakeTextLowercase{\thesubsubsection}}}{1em}{\normalsize\itshape} 


% dual glossary and acronym entries, see: https://en.wikibooks.org/wiki/LaTeX/Glossary
%\usepackage[xindy,toc,acronym]{glossaries}
\usepackage[acronym,toc,xindy]{glossaries-extra}
%\setabbreviationstyle[acronym]{long-short-sc}
%\GlsAddXdyLocation{negativepage}{:sep "-" "arabic-numbers"}
\usepackage{xparse}
% acronym print style - requires glossaries-extra version: 2017/11/03 v1.21 (NLCT)
\newglossarystyle{acronymsee}{
    \setglossarystyle{long}% base this style on the list style\renewcommand{\subglossentry}[3]{%
    \renewcommand{\glossentry}[2]{%
        \glsentryitem{##1}\glstarget{##1}{\glossentryname{##1}} &\!\!\!\!\glsxtrusesee{##1}\tabularnewline%
        %\glsentryitem{##1}\glstarget{##1}{\glossentryname{##1}} &##2\tabularnewline%
    }%
}
% glossary entries w/acronyms
\DeclareDocumentCommand{\newdualentry}{ O{} O{} m m m } {
	\newglossaryentry{gls-#3}{name={#4},text={#4\glsadd{#3}},
		description={#5},#1
	}
	\makeglossaries
    \newacronym[see={[]{gls-#3}},#2]{#3}{#3}{#4\glsadd{gls-#3}}
}
\DeclareDocumentCommand{\newdualentrysee}{ O{} O{} m m m m } {
    \newglossaryentry{gls-#3}{name={#4},text={#4\glsadd{#3}},
    	description={#5},#1,
    	see={[see also:]{#6}}
    }
    \makeglossaries
    \newacronym[see={[]{gls-#3}},#2]{#3}{#3}{#4\glsadd{gls-#3}}
}
\DeclareDocumentCommand{\newsingleentry}{ O{} O{} m m m } {
	\newglossaryentry{#3}
	{
		name=#4,
		description={#5}
	}
	\makeglossaries
}
\DeclareDocumentCommand{\newsingleentrysee}{ O{} O{} m m m m } {
    \newglossaryentry{#3}
    {
    	name=#4,
    	description={#5},
    	see={[see also:]{#6}}
    }
    \makeglossaries
}

% for chapter dependency diagram
\newcommand{\chapternode}[4]{
	\node (#1) [#2] {\textbf{Chapter \ref{#3}:} \\ #4};
}
\newcommand{\chapternodeat}[4]{
\node (#1) at (#2) {\textbf{Chapter \ref{#3}:} \\ #4};
}

% customizations
\definecolor{matDB}{HTML}{352A87}
\definecolor{matLB}{HTML}{0D75DC}
\definecolor{matTK}{HTML}{07a9c2}
\definecolor{matGE}{HTML}{7CBF7B}
\definecolor{matDB}{HTML}{352A87}
\definecolor{matOR}{HTML}{F1B94A}
\definecolor{matYE}{HTML}{F9FB0E}

% tikz labels from table file
\makeatletter
\pgfplotsset{
	/pgfplots/flexible xticklabels from table/.code n args={3}{%
		\pgfplotstableread[#3]{#1}\coordinate@table
		\pgfplotstablegetcolumn{#2}\of{\coordinate@table}\to\pgfplots@xticklabels
		\let\pgfplots@xticklabel=\pgfplots@user@ticklabel@list@x
	}
}
\makeatother
\usetikzlibrary{pgfplots.groupplots}
\pgfplotsset{
	select row/.style={
		x filter/.code={\ifnum\coordindex=#1\else\def\pgfmathresult{}\fi}
	}
}


==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

In our earlier work \cite{Paulini-MultiBitAllocation-Odyssey-2016}, we elaborated on biometric template protection schemes for speaker recognition: voice reference in terms of Gaussian mixture model (GMM) supervectors, which are binarized, such that standardized protection schemes can be employed \cite{ISO-IEC-24745-TemplateProtection-101129}.
Contrary to \cite{Vaquero-VoiceBTP-Interspeech-2015}, motivating no need for template protection depending on the feature extraction, ISO/IEC~24745 \cite{ISO-IEC-24745-TemplateProtection-101129} further requires \emph{unlinkability}. Linkability of state\-/of\-/the\-/art speaker recognition features is demonstrated in \cite{Glembek-MigratingIvectors-Interspeech-2015}, especially with the motivation of interchanging features among different voice biometric services.
The interchange of biometric data across services is recently addressed ethically in \cite{Moyakine-SIIPPanelEthics-EABrpc-2017}, especially when targeting forensic and investigatory scenarios. Accounting for latest data privacy legislations, we motivate template protection, especially in commercial scenarios, but also in other dual\-/use applications.

Related work on the binarization of traditional speaker recognition systems employing universal background models (UBMs) targeting the GMM\,--\,UBM approach can be found in \cite{AngueraBonastre-SpeakerBinaryKey-Interspeech-2010,Bonastre-DiscriminantBinaryData-ICASSP-2011,Hernandez-SpeakerBinaryRepresentation-ProgressPatternRecognition-2012}.
However, due to the binarization process, the biometric performance usually declines, and calibration properties are lost.
Contrary to performance\-/lossy template protection approaches as biometric cryptosystems and cancelable biometrics~\cite{Rathgeb-BTP-Survey-EURASIP-2011}, HE completely preserves biometric accuracy. 
Therefore, we investigate on Paillier HE schemes
% in order to sustain score properties \cite{GomezBarrero-MBTPwithHE-PR-2017,GomezBarrero-VariableLengthBTPHE-Access-2017}
, which are already introduced to other biometric modalities, such as signature~\cite{gomez2016implementation}, iris~\cite{penn2014customisation}, and fingerprint~\cite{barniprivacy} recognition, considering Hamming distances (XOR operator), dynamic time warping (DTW), the Euclidean distance, and the cosine similarity.
Targeting data privacy, biometric template protection schemes need to fulfill ISO/IEC~24745~\cite{ISO-IEC-24745-TemplateProtection-101129} requirements:
\begin{itemize}
    \item \emph{unlinkability}: stored biometric templates shall not be linkable across applications or databases (\emph{cross-matching}),
    \item \emph{irreversibility}: biometric samples cannot be reconstructed from encrypted biometric templates,
    \item \emph{renewability}: multiple biometric references can be independently transformed, when they are created from one or more samples of a biometric data capture subject.
\end{itemize}
\todo[inline]{this is far too brief, however do we need more detail on Binary Template Protection? No favor of mine ...}

\subsection{Homomorphic Cryptosystems}
Homomorphic encryption~\cite{Rivest-PrivacyHomomorphisms-SecureComputation-1978,FontaineGaland-Survey-HomomorphicEncryption-JIS-2007,Hoffstein-IntroductionCryptography-2008} has the property that computations on the ciphertext directly affect the plaintext.
Homomorphisms are functions, which preserve algebraic structures of groups \cite{Hungerford-Algebra-Springer-1974}.
The function $f: G \rightarrow H$ is a homomorphism for groups $(G, \diamond), (H, \smallsquare)$ with sets $G, H$ and operators $\diamond, \smallsquare$ if:
\begin{equation}
f(g \diamond g') = f(g) \smallsquare f(g') \qquad \forall g,g' \in G.
\end{equation}

Public-key cryptosystems $(K, M, C, \enc, \dec)$ with sets of keys $K$, plaintexts $M$, ciphertexts $C$, and sets of functions representing encryption $\enc$ and decryption $\dec$ are homomorphic if:
\begin{align}
\forall m_1,m_2 \in M, &\forall e \in K: \\\nonumber
\enc_e(m_1) \smallsquare \enc_e(m_2) &= \enc_e(m_1 \diamond m_2)
\end{align}
where public keys $e$ specify encryption and private keys $d$ decryption functions, respectively:
\begin{align}
\enc_e: M \rightarrow C,\qquad \dec_d: C \rightarrow M.
\end{align}

\subsubsection{Brief Summary: HE in Biometrics}
In \cite{Barni-BTP-SPM-2015} and \cite{Bringer-BTP-Survey-SPM-2013}, the authors provide an overview of several biometric template protection schemes based on homomorphic encryption and garbled circuits. Barni et al.~\cite{barniprivacy} present a way to protect fixed-length fingercodes~\cite{Jain-Fingercodes-IEEE-1997} using homomorphic encryption. This system was modified in \cite{Bianchi-BTP-Fingercode-BIOMS-2010} to accelerate the process by reducing the size of the fingercode. However, a reduction of information always leads to a degradation of biometric accuracy. 
Ye et al. present an anonymous biometric access control (ABAC) system~\cite{Ye-BTP-HE-EURASIP-2009} for iris recognition. Their system setup verifies only whether a subject is enrolled without revealing the identity and thus grants anonymity towards the subjects. Another ABAC protocol is proposed in \cite{Luo-BTP-HE-ICME-2009} by Luo \mbox{et al.} and a secure similarity search algorithm is presented for anonymous authentication.
Combining homomorphic encryption with garbled circuits, Blanton and Gasti~\cite{Blanton-BTP-IrisFingerprint-ESORICS-2011} implement secure protocols for iris and fingerprint recognition.

Encryption algorithms based on lattices are found to be post-quantum secure~\cite{quantum} which is a convenient property for a public key encryption scheme. 
Using ideal lattices in a somewhat homomorphic 	encryption (SHE) scheme, Yasuda et al.~\cite{Yasuda-BTP-HE-ARES-2013} compute the Hamming distance of encrypted templates in an efficient way by using a packing method before the encryption.
Using binary feature vectors with constant size of 2048 bits for every biometric data, again Yasuda et al.~\cite{Yasuda-BTP-HE-SCN-2015} present a new packing method in a SHE scheme for biometric authentication based on a special version of the ring-LWE assumption.
Another privacy-preserving biometric authentication approach~\cite{Patsakis-BTP-HE-DPM-2015} splits a 2048 bits iris code into 64 blocks with 32 bits each and encrypts these blocks using the lattice-based encryption scheme NTRU. As in the aforementioned works, they compute the distance in the encrypted domain never disclosing biometric data.


\subsubsection{Paillier HE Scheme}
Motivated by \cite{gomez2016implementation,GomezBarrero-VariableLengthBTPHE-Access-2017,GomezBarrero-MBTPwithHE-PR-2017}, this work puts emphasis on the asymmetric Paillier cryptosystems \cite{paillier1999public,Zhu-PrivacyPreservingTimeSeriesData-EDBT-2014}, a homomorphic probabilistic encryption scheme based on the decisional composite residuosity assumption (DCRA): for integers $n,z$ it is hard to decide, whether $z$ is an $n$-residue modulo $n^2$.
Due to the DCRA, Paillier cryptosystems are secure against \emph{honest but curious users} conducting chosen ciphertext attacks \cite{paillier1999public,bellare1998relations,paillier1999efficient}.
In Paillier cryptosystems, the public key $e = (n,g)$ is defined by $n = p\,q$ and $g\in\Z^*_{n^2}$, where $p,q$ are two large prime numbers, such that $\gcd(p\,q,(p-1)\,(q-1)) = 1$, and with $\Z^*_{n^2}$ as the set of module $n^2$ integers having a multiplicative inverse.
Based on $p,q$, the secret key $sk = (\lambda, \mu)$ is defined by $\lambda = \lcm(p-1,q-1)$ and $\mu = \left(g^{\lambda} \mod n^2\right)^{-1} \mod n$.

During encryption $c = \enc_e(m,s) \in \Z^*_{n^2}$ of a message $m\in\Z_n$ with public key $e$, a random number $s \in \Z^*_n$ sustains the probabilistic nature of the cryptosystem, \ie $\enc_e(m, s_1) \neq \enc_e(m, s_2)$ for two different $s_1,s_2 \in \Z^*_n$:
\begin{equation}
c = \enc_e(m,s) = g^m\,s^n \mod{n^2},
\end{equation}
which is abbreviated in the following as $\enc_e(m)$, whereas ciphertexts are decrypted as:
\begin{equation}
m' = \dec_d(c) = \frac{\left(c^{\lambda} \mod{n^2}\right) - 1}{n}\,\mu \mod{n}.
\end{equation}
Assuming no cryptographic errors, $m' = m$, as such in the following.
Similarly to \cite{gomez2016implementation,GomezBarrero-VariableLengthBTPHE-Access-2017,Zhu-PrivacyPreservingTimeSeriesData-EDBT-2014,GomezBarrero-MBTPwithHE-PR-2017}, we utilize the additive homomorphic properties of the Paillier cryptosystem regarding plaintexts $m_1,m_2$ and corresponding ciphertexts $c_1,c_2$:
\begin{align}
\dec_d\left(c_1\,c_2\right) &= m_1 + m_2 \mod{n},\nonumber\\
\dec_d\left({c_1}^l\right) &= m_1\,l \mod{n}, \emph{ with a constant l}.
\label{eq:HE:properties}
\end{align}
In other words, whereas the decrypted product of two ciphertexts resembles as the sum of two plaintexts, the decrypted exponentiation of a ciphertext results in the product of the depending plaintext and exponent.
In the following, we substitute for public key instances $pk, pk1, pk2$ for $e$, and secret key instances $sk, sk1, sk2$ for $d$, respectively.

\subsection{Homomorphic Template Protection}
Targeting biometric template protection, data privacy friendly comparison schemes are sought, in which encrypted references are stored in databases rather than plaintext.
As such, the Euclidean and cosine similarity comparison scores $S_{\emph{Euc}}, S_{\emph{cos}}$ between two F-dimensional vectors $\bm{X} = \{x_1, \dots, x_F\}, \bm{Y} = \{y_1, \dots, y_F\}$ are computationally derived as \cite{gomez2016implementation,GomezBarrero-VariableLengthBTPHE-Access-2017,GomezBarrero-MBTPwithHE-PR-2017}:
\begin{align}
S_{\emph{Euc}}\left(\bm{X}, \bm{Y}\right) &= \sum\limits_{f=1}^F x_f^2 + \sum\limits_{f=1}^F y_f^2 - 2\,\sum\limits_{f=1}^F x_f\,y_f,\nonumber\\
\enc_{pk}\left(S_{\emph{Euc}}\left(\bm{X}, \bm{Y}\right)\right) &= \enc_{pk}\left(\sum\limits_{f=1}^F x_f^2\right)\,\enc_{pk}\left(\sum\limits_{f=1}^F y_f^2\right)\nonumber\\
&\hphantom{{}={}}\prod\limits_{f=1}^F\enc_{pk}\left(y_f\right)^{-2\,x_f},
\end{align}
with the protected reference:
\begin{equation}
\Bigg(\enc_{pk}\left(\sum\limits_{f=1}^F y_f^2\right), \left\{\enc_{pk}\left(y_f\right)\right\}_{f=1}^F\Bigg),
\end{equation}
where for this work the cosine comparison is of more relevance:
\begin{align}
S_{\emph{cos}}\left(\bm{X}, \bm{Y}\right) &= \frac{\bm{X}\cdot\bm{Y}}{||\bm{X}||\,||\bm{Y}||} = \sum\limits_{f=1}^F\frac{x_f\,y_f}{||\bm{X}||\,||\bm{Y}||},\nonumber\\
\enc_{pk}\left(10^{^{12}}\,S_{\emph{cos}}\left(\bm{X}, \bm{Y}\right)\right) &= \prod\limits_{f=1}^F\enc_{pk}\left(\frac{10^6\,y_f}{||\bm{Y}||}\right)^{\frac{10^6\,x_f}{||\bm{X}||}},
\end{align}
with the protected reference:
\begin{equation}
\left(\left\{\enc_{pk}\left(\frac{10^6\,y_f}{||\bm{Y}||}\right)\right\}_{f=1}^F\right),
\end{equation}
with scaling factor $10^{12}$ for the purpose of sustaining a broader range of integer values representing positive float values extracted from \eg, biometric signature samples.

\begin{figure}[htb]
    \centering
%    \includegraphics[width=1\linewidth]{figures/HE_2Cov/diagram_cosine.pdf}
    \input{figures/HE_2Cov/arch_cos.tex}
    \caption{Architecture of homomorphic encrypted cosine similarity comparison, \cf~\cite{gomez2016implementation}, with client, servers (blue) and communication channels (orange).}
    \label{fig:cos_arch}
\end{figure}

Fig.~\ref{fig:cos_arch} illustrates a distributed client\,--\,server architecture employing HE in cosine comparison: a client $C$ extracts the probe feature vector $\bm{X}$ and requests the encrypted reference feature vector $enc_{pk}(\bm{Y})$ from the database $\mathrm{DB}_{\emph{subject}}$, scores are calculated on the client, and send to the authentication server $\mathrm{AS}_{\emph{subject}}$, holding the key pair $(pk, sk)$ for the following decryption of the score. Based on pre-defined threshold, $\mathrm{AS}_{\emph{subject}}$ outputs the decision $D$ of whether the decrypted score $S_{\emph{cos}}$ exceeds a threshold~$\eta$ or not.
Tab.~\ref{tab:complexityRelated} provides an overview to the complexity of the encrypted Euclidean and cosine comparison, where numbers diverge from \cite{gomez2016implementation} as in the signature recognition scenario, five reference templates are encrypted rather than \eg, an averaged template model.
As references are encrypted during enrollments, cosine verifications require no additional encryptions, whereas Euclidean distance comparators require probe encryptions.

\begin{table}[htb]
    \caption{Complexity analysis for the Euclidean and cosine comparators during verification, \cf \cite{gomez2016implementation}, assuming $F=250$ dimensional features, the size of an encrypted feature $c=0.5\KiB$, and the plain feature size $p=64\bit$.}
    \label{tab:complexityRelated}
    \scriptsize
    \centering
    \smallskip
    \begin{tabular}{lcc} % {p{2.9cm}P{1.6cm}P{2.375cm}P{3.125cm}} 
        \toprule
        & Euclidean & Cosine \\
        \midrule
        N$^o$ encryptions & $1$ & $0$\\
        N$^o$ decryptions & $1$ & $1$\\
        \midrule
        N$^o$ additions & $F-1$ & $0$ \\
        N$^o$ products & $2\,F+4$ & $F - 1$ \\
        N$^o$ exponentiations & $2\,F$ & $F$ \\
        \midrule
        Plain template size & $p\,F$ & $p\,F$ \\
        & $\approx 2.0\KiB$  & $\approx 2.0\KiB$ \\
        Protected template size & $c\,(F+1)$ & $c\,F$ \\
        & $= 125.5\KiB$ & $= 125.0\KiB$ \\
        %        \midrule
        %        Plain model size & $0$ & $0$ \\
        %        & $=0.0\KiB$ & $=0.0\KiB$ \\
        %        Protected model size & $0$ & $0$ \\
        %        & $=0.0\KiB$ & $=0.0\KiB$ \\
        \midrule
        Channels: amount of & $c\,(F+2)$ & $c\,(F + 1)$ \\
        protected data exchanged & $= 126.0\KiB$ & $= 125.5\KiB$ \\
        \bottomrule
    \end{tabular}
\end{table}

Motivated by the HE schemes for integer vectors, we target the computation of probabilistic comparison scores employing the (symmetric) dot product:
\begin{align}
\enc_{pk}(\bm{Y})^{\bm{X}} &= \prod\limits_{f=1}^F(y_f)^{x_f} = \enc_{pk}(\bm{X}\cdot\bm{Y}) \nonumber\\
& = \prod\limits_{f=1}^F(x_f)^{y_f} = \enc_{pk}(\bm{X})^{\bm{Y}}.
\label{eq:HE:dotproduct}
\end{align}

\subsection{Speaker Recognition: Two-Covariance Comparator}
Recent speaker recognition approaches rely on intermediate\-/sized vectors (i-vectors), representing the characteristic speaker offset from a UBM, which models the distribution of acoustic features, such as Mel-Frequency Cepstral Coefficients (MFCCs) \cite{Reynolds-GMMs-ConversationalSpeech-2000}.
Thereby, UBM components' mean vectors are concatenated to a \emph{supervector} $\bm{\mu_{\text{UBM}}}$.
Speaker supervectors \(\bm{s}\) are decomposed by a total variability matrix $\mathbf{T}$ into a lower-dimensional and higher-discriminant i\-/vectors $\bm{i}$ as an offset to the UBM supervector $\bm{\mu_{\text{UBM}}}$:
\begin{align}
    \label{eq:ivec}
    \bm{s} = \bm{\mu_{\text{UBM}}} + \bm{T}\,\bm{i}.
\end{align}
The total variability matrix is trained on a development set using an expectation maximization algorithm \cite{Dehak-FrontEndFactorAnalysis-ivector-TASLP-2011,Kenny-JFA-Theory-CRIM-2005}. 
Then, \mbox{i-vectors} are projected onto a spherical space by whitening transform and length-normalization \cite{GarciaRomeroEpsyWison-ivector-lengthnormalization-Interspeech-2011,Bousquet-BenefitsDifferentSteps-ivectors-CIARP-2013}.

State-of-the-art \mbox{i-vector} comparators belong to the PLDA family \cite{Cumani-GenerativePairwiseModels-Odyssey-2014,Bousquet-BenefitsDifferentSteps-ivectors-CIARP-2013}.
PLDA comparators conduct a likelihood ratio scoring comparing the probabilities of the hypotheses (a) reference and probe \mbox{i-vectors} $\bm{X}, \bm{Y}$ stem from the same source, or (b) stem from different sources. 
Therefore, speaker within and between variabilities are examined in a latent feature subspace.
In this work, emphasis is put on the 2Cov approach \cite{Cumani-PairwiseDiscriminativeVerification-TASLP-2013,Cumani-GenerativePairwiseModels-Odyssey-2014}, the full\-/subspace Gaussian PLDA.
The closed-form solution to the 2Cov scoring is denoted regarding within and between covariances $\bm{W}, \bm{B}$ with mean $\bm{\mu}$ \cite{Cumani-PairwiseDiscriminativeVerification-TASLP-2013}, resulting in the log\-/likelihood ratio score $S_{\emph{2Cov}}$:
\begin{align}
    S_{\emph{2Cov}}\left(\bm{X}, \bm{Y}\right) &= 
    \bm{X'}\,\bm{\Lambda}\,\bm{Y} + \bm{Y'}\,\bm{\Lambda}\,\bm{X}+ \bm{X'}\,\bm{\Gamma}\,\bm{X} + \bm{Y'}\,\bm{\Gamma}\,\bm{Y} + \nonumber\\
    &\hphantom{{} = {}} \bm{c'}\,\left(\bm{X} + \bm{Y}\right) + k,\nonumber\\
    \textit{with: } \bm{\Lambda} &= \frac{1}{2}\bm{W'}\,\bm{\tilde{\Lambda}}\,\bm{W},
    \quad
    \bm{\Gamma} = \frac{1}{2}\bm{W'}\,\left(\bm{\tilde{\Lambda}}-\bm{\tilde{\Gamma}}\right)\,\bm{W},\nonumber\\
    \bm{c} &= \bm{W'}\,\left(\bm{\tilde{\Lambda}}-\bm{\tilde{\Gamma}}\right)\,\bm{B}\,\bm{\mu},
    \nonumber\\
    k &= \tilde{k} + \frac{1}{2}\left(\left(\bm{B}\,\bm{\mu}\right)'\,\left(\bm{\tilde{\Lambda}} - 2\,\bm{\tilde{\Gamma}}\right)\,\bm{B}\,\bm{\mu}\right),\nonumber\\
    \bm{\tilde{\Lambda}} &= \left(\bm{B} + 2\,\bm{W}\right)^{-1},
    \quad
    \bm{\tilde{\Gamma}} = \left(\bm{B}+\bm{W}\right)^{-1},\nonumber\\
    \tilde{k}&= 2\,\log|\bm{\tilde{\Gamma}}| - \log|\bm{\tilde{\Lambda}}| - \log|\bm{B}| + \bm{\mu'}\,\bm{B}\,\bm{\mu}.
    \label{eq:HE:2CovCumani}
\end{align}

